Concept Activation Regions: A Generalized Framework For Concept-Based Explanations

Concept-based explanations permit to understand the predictions of a deep neural network (DNN) through the lens of concepts specified by users. Existing methods assume that the examples illustrating a concept are mapped in a fixed direction of the DNN's latent space. When this holds true, the concept can be represented by a concept activation vector (CAV) pointing in that direction. In this work, we propose to relax this assumption by allowing concept examples to be scattered across different clusters in the DNN's latent space. Each concept is then represented by a region of the DNN's latent space that includes these clusters and that we call concept activation region (CAR). To formalize this idea, we introduce an extension of the CAV formalism that is based on the kernel trick and support vector classifiers. This CAR formalism yields global concept-based explanations and local concept-based feature importance. We prove that CAR explanations built with radial kernels are invariant under latent space isometries. In this way, CAR assigns the same explanations to latent spaces that have the same geometry. We further demonstrate empirically that CARs offer (1) more accurate descriptions of how concepts are scattered in the DNN's latent space; (2) global explanations that are closer to human concept annotations and (3) concept-based feature importance that meaningfully relate concepts with each other. Finally, we use CARs to show that DNNs can autonomously rediscover known scientific concepts, such as the prostate cancer grading system.

==> Parts/car_counterfactual.tex <==
\textbf{Counterfactual explanations.} Beyond feature importance, another class of explanation method involving features are counterfactual explanations~\cite{Wachter2017}. Those explanations find the minimal modification of the features $\x$ that causes the prediction $\f(\x)$ to change (for instance the predicted class flips). By exploiting the concept sets densities, it is perfectly possible to apply a similar approach to increase or decrease the concept density of an input $\x$. For instance, if the concept density $\rho^c[\g(\x)]$ is low, one could construct a sparse perturbation $\pert \in \R^{d_X}$ of the features that increases the concept density by solving $\arg \max_{\pert \in \R^{d_X}} \left[ \rho^{\Pos^c}[\g(\x + \pert)] - \lambda \norm[1]{\pert} \right]$, where $\norm[1]{\cdot}$ denotes the $l^1$ norm and the parameter $\lambda \in \R^+$ controls the sparsity of the perturbation. In a similar way, one can construct a perturbation that decreases the concept density by replacing $\rho^{\Pos^c}$ with $\rho^{\Neg^c}$. Note that, in both cases, these perturbations can be obtained with gradient-based optimizers if the black-box and the kernel function are differentiable. We note that both of these perturbations move the initial representation $\g(\x)$ to another representation $\g(\x + \pert)$ that is located in a region of $\H$ with a higher density of positive or negative examples related to the concept of interest. In both cases, the perturbed representation $\g(\x + \pert)$ is therefore unlikely to land in an region of $\H$ that is out of distribution. \hl{Verify empirically and contrast with the original TCAV paper.} 
